Thermodynamic Bifurcations of Boiling in Solid-State Nanopores

Boiling heat transfer is the basis of many commonly used cooling techniques. In cooling of electronic devices, for example, it is desirable to further miniaturize heat exchangers to achieve higher heat transfer, and thus it is necessary to understand boiling phenomena on shorter spatial and temporal scales. This is especially challenging at the nanometer scale because conventional imaging techniques cannot capture the dynamics of nanobubbles, owing to the Abbe diffraction limit. Here in this research, we utilize the nanopore Joule heating system that enables the generation of nanobubbles and simultaneous diagnosis of their nanosecond resolution dynamics using resistive pulse sensing. When a bias voltage is applied across a silicon nitride nanopore immersed in an aqueous salt solution, Joule heat is generated owing to the flow of ionic current. With increasing voltage, the Joule heating intensifies, and the temperature and entropy production in the pore increase. Our sensing results show that nanopore boiling follows the theory of minimum entropy production and attempts to settle to a minimum dissipative state. This results in two boiling bifurcations corresponding to the transition between different boiling states. These characteristics of nanopore boiling are represented by an "M"-shaped boiling curve, experimentally obtained from the Joule heat variation with the applied voltage. A theoretical framework is proposed to model the thermodynamics of nanopore bubbles and estimate the system dissipation which explains the four arms of the "M"-shaped boiling curve. The present study reveals that the utilization of nanopore boiling as a benchmark platform offers a valuable means for investigating the intricate boiling phenomenon and its correlation with nanoscale bubble dynamics. This would provide fundamental insights into the chaotic transition boiling regime, which is least understood.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );
        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );
        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> xx.tex <==


